Anonymous Self-Stabilising Localisation via Spatial Population Protocols

In the distributed localization problem (DLP), $n$ anonymous robots (agents) $a_0, a_1, ..., a_{n-1}$ begin at arbitrary positions $p_0, ..., p_{n-1}$ in $S$, where $S$ is an Euclidean space. The primary goal in DLP is for agents to reach a consensus on a unified coordinate system that accurately reflects the relative positions of all points, $p_0, ..., p_{n-1}$. Extensive research on DLP has primarily focused on the feasibility and complexity of achieving consensus when agents have limited access to inter-agent distances, often due to missing or imprecise data. In this paper, however, we examine a minimalist, computationally efficient model of distributed computing in which agents have access to all pairwise distances, if needed. Specifically, we introduce a novel variant of population protocols, referred to as the spatial population protocols model. In this variant each agent can memorise one or a fixed number of coordinates, and when agents $a_i$ and $a_j$ interact, they can not only exchange their current knowledge but also either determine the distance $d(i,j)$ between them in $S$ (distance query model) or obtain the vector $v(i,j)$ spanning points $p_i$ and $p_j$ (vector query model). We propose several localisation protocols, including: (1) Two leader-based protocols with distance queries, stabilizing silently in $o(n)$ time using an efficient multi-contact epidemic, a generalization of the one-way epidemic in population protocols; (2) A distance-based protocol self-stabilizing silently in $O(n(\log n/n)^{1/(k+1)}\log n)$ time in $k$-dimensions, leveraging a leader election mechanism; (3) An optimally fast protocol with vector queries, self-stabilizing silently in $O(\log n)$ time.

==> ar-abstract_for_submisssion.tex <==
In the distributed localization problem (DLP), n anonymous robots (agents) A1, ..., An begin at arbitrary positions x1, ..., xn in an Euclidean space. Initially, each agent Ai operates within its own coordinate system, which may be inconsistent with those of other agents. The primary goal in DLP is for agents to reach a consensus on a unified coordinate system that accurately reflects the relative positions of all points, p1, ..., pn. Extensive research on DLP has primarily focused on the feasibility and complexity of achieving consensus when agents have limited access to inter-agent distances, often due to missing or imprecise data. In this paper, however, we examine a minimalist, computationally efficient model of distributed computing in which agents have access to all pairwise distances, if needed. Specifically, we introduce a novel variant of population protocols, referred to as the spatial population protocols model. In this variant each agent can memorise one or a fixed number of coordinates, and when agents Ai and Aj interact, they can not only exchange their current knowledge but also either determine the distance  between them in (distance query model) or obtain the vector spanning points pi and pj (vector query model).
We propose and analyse several distributed localisation protocols, including:
1. Leader-based localisation protocol with distance queries
We propose and analyse two leader-based localisation protocols that stabilize silently in o(n) parallel time. These protocols leverage an efficient solution to the novel concept of multi-contact epidemic, a natural generalisation of the core communication tool in population protocols, known as the one-way epidemic.
2. Self-stabilising leader localisation protocol with distance queries. We show how to effectively utilise a leader election mechanism within the leader-based localisation protocol to get DLP protocol that self-stabilises silently in parallel time O(n(log n/n)^{1/(k+1)} log n) in k-dimensions. 
3. Self-stabilising localisation protocol with vector queries. 
We propose and analyse an optimally fast DLP protocol which self-stabilises silently in O(log n) parallel time.

We conclude with a discussion on future research directions for distributed localisation in spatial population protocols, including scenarios that account for higher dimensions, limited precision and susceptibility to errors. 
A brief announcement with partial results of this paper will appear in SAND 2025.

==> ar-algPosK.tex <==

\begin{algorithm}
\caption{Positioning in $k$ dimensions}
\label{alg:Pos_k}
\Begin{
    $i=0; C[leader]=\texttt{green}$;\\
    \While{i<k}{
        during an interaction between agents $A_u$ and $A_v$\;
        \If{$(A_u$ is $leader) \wedge (C[A_v]=\texttt{blue})$}
        {
        \If{$A_v$ interacted with all $i$ \texttt{green} agents}
        {position $A_v$ and stabilise $h_v$;\\ $C[A_v]=\texttt{green}$; \\$i=i+1$}
    }
    %$C[A_u]=\texttt{green}$;
  }
    \While{not all agents are positioned}{
        during an interaction between agents $A_u$ and $A_v$\;
        \If{$(C[A_u]=\texttt{green}) \wedge (C[A_v]=\texttt{blue})$}
        {
        \If{$A_v$ interacted with $k+1$ distinct green agents}
        {position $A_v$ and stabilise $h_v$;\\ $C[A_v]=\texttt{green}$}
    }
  }
}
\end{algorithm}

